A Second-Order Approach to Complex Event Recognition

Complex Event Recognition (CER for short) refers to the activity of detecting patterns in streams of continuously arriving data. This field has been traditionally approached from a practical point of view, resulting in heterogeneous implementations with fundamentally different capabilities. The main reason behind this is that defining formal semantics for a CER language is not trivial: they usually combine first-order variables for joining and filtering events with regular operators like sequencing and Kleene closure. Moreover, their semantics usually focus only on the detection of complex events, leaving the concept of output mostly unattended. In this paper, we propose to unify the semantics and output of complex event recognition languages by using second order objects. Specifically, we introduce a CER language called Second Order Complex Event Logic (SO-CEL for short), that uses second order variables for managing and outputting sequences of events. This makes the definition of the main CER operators simple, allowing us to develop the first steps in understanding its expressive power. We start by comparing SO-CEL with a version that uses first-order variables called FO-CEL, showing that they are equivalent in expressive power when restricted to unary predicates but, surprisingly, incomparable in general. Nevertheless, we show that if we restrict to sets of binary predicates, then SO-CEL is strictly more expressive than FO-CEL. Then, we introduce a natural computational model called Unary Complex Event Automata (UCEA) that provides a better understanding of SO-CEL. We show that, under unary predicates, SO-CEL captures the subclass of UCEA that satisfy the so-called *-property. Finally, we identify the operations that SO-CEL is lacking to capture UCEA and introduce a natural extension of the language that captures the complete class of UCEA under unary predicates.

==> expressiveness.tex <==
%!TEX root = ../main/main.tex

After proving that all CEPL formulas with unary predicates can be translated into match automata, it is natural to ask whether this holds in the other direction, namely, if every MA can be translated into an equivalent CEPL formula with unary predicates.
If we restrict to core-CEPL, then the answer is no, mainly because MA can take decisions based on tuples that are not part of the output match, while formulas in core-CEPL cannot.
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[->,>=stealth, 
		semithick, 
		auto,
		initial text= {},
		initial distance= {3mm},
		accepting distance= {4mm},node distance=3.3cm, semithick]
		\tikzstyle{every state}=[draw=black,text=black,inner sep=0pt, minimum size=8mm]
		
		
		\node[initial,state]	(1) 				{$q_1$};
		\node[state]			(2) [right of=1]	{$q_2$};
		\node[accepting,state]	(3) [right of=2]	{$q_3$};
		
		\path
		(1) edge 				node {$\type(x) = T \mid \umark$} (2)
		edge [loop above] 	node {$\TRUE \mid \umark$} (1)
		(2) edge [loop above] 	node {$\TRUE \mid \umark$} (2)
		edge 				node {$\type(x) = H \mid \amark$} (3);
		\end{tikzpicture}
		\caption{A match automaton that is not equivalent to any core-CEPL formula.}\label{fig:ma-coreCEPL}
	\end{center}
\end{figure}
As an example, consider the MA in Figure~\ref{fig:ma-coreCEPL} that returns the matches that consist of a single $H$-tuple and there exists another $T$-tuple before the $H$-tuple which is not part of the match.
Clearly, there is no formula in core-CEPL that is equivalent to the match automaton above.

In order to capture the exact expressiveness of core-CEPL, we restrict MA to a new semantics that we called the \emph{$*$-semantics}.
%The difference of the semantics is in the way the automaton runs.
Formally, let $\cA = (Q, \Delta, I, F)$ be a match automaton and $S=t_1,t_2,\ldots$ be a stream.
A $*$-run $\rho$ of $\cA$ over $S$ is a sequence of transitions:
$$
\rho: (q_0,0) \ \trans{\alpha_1} \ (q_1,i_1) \  \trans{\alpha_2} \ \cdots \ \trans{\alpha_n} (q_n,i_n)
$$
such that $q_0 \in I$, $0 < i_1 < \ldots < i_n$ and, for every $j \geq 1$, $(q_{j-1}, \alpha_j, \amark, q_j) \in \Delta$ and $S[i_j] \models \alpha_j$.
We say that $\rho$ is an accepting $*$-run if $q_n \in F$.
Furthermore, we denote by $\rmatch(\rho) = \{i_1, \ldots, i_n\}$, and define the set of all matches of $\cA$ over $S$ under the $*$-semantics as:
$
\ssem{\cA}(S) = \{\rmatch(\rho) \mid \text{$\rho$ is an accepting $*$-run of $\cA$ over $S$} \}
$.
Notice that the automaton no longer has the ability to verify a condition on a tuple with an unmarked position.
Indeed, one may eliminate the marking symbols on the transitions, i.e., consider $\Delta \subseteq Q \times \fset_u(\cR) \times Q$.
For the sake of simplicity, we keep the syntax of MA and just restrict its semantics instead of defining a new automata model.

%A basic property of this semantics is that for every MA $\cA$, there is another MA $\cA'$ such that $\sem{\cA}_*(S) = \sem{\cA'}(S)$ for every stream $S$.
%Basically, $\cA'$ is the result of adding the $\amark$ mark to every transition of $\cA$ and a loop with $\umark$ and $true$ condition for every state. Formally, if $\cA=(Q,\Delta,I,F)$ then $\cA'=(Q,\Delta',I,F)$ where $\Delta'=\{(p,(\alpha,\amark),q) \mid (p,\alpha,q)\in \Delta\} \cup \{(q,(true,\umark),q) \mid q\in Q \}$.

With the new semantics, we can effectively capture the expressiveness of unary core-CEPL as follows.
\begin{theorem} \label{theo:CEP_MA*}
	Core-CEPL with unary predicates is equally expressive as MA under the $*$-semantics, namely, for every core-CEPL formula $\varphi$ with unary predicates, there exists a MA $\cA$ such that $\sem{\varphi}(S)=\ssem{\cA}(S)$ for every stream $S$, and conversely.
\end{theorem}
%The proof for the first part is similar to the one in section~\ref{section}. Basically, $\varphi$ is first translated into normal form and then the automaton $\cA$ is constructed recursively.
%The proof for the second part follows the same idea as the proof that FSA can be expressed as regular expressions.
%For the sake of saving space, the complete proof for Theorem~\ref{theo:CEP_MA*} has been moved to the appendix.

Theorem~\ref{theo:CEP_MA*} gives a useful result for the study of core-CEPL with unary predicates, since it provides the exact computational model to analyze the core fragment of CEPL.
Moreover, statements resulting from the study of MA under $*$-semantics can be further applied to core-CEPL with unary predicates and conversely.

An interesting property of the $*$-semantics is that, for every MA $\cA$, stream $S$, and match $M \in \ssem{\cA}(S)$, we can arbitrarily modify, add or remove tuples in $S$ that are not \emph{marked} by~$M$, and the original tuples in $M$ would still make a match of~$\cA$ over the resulting stream.
To formalize this, we need some additional definitions.
A \emph{match-function} $f$ is a function $f:\streams(\cR) \rightarrow 2^\mset$, where $\streams(\cR)$ is the set of all $\cR$-streams and $\mset$ is the set of all matches (i.e. the set of all finite subsets of $\bbN$).
Although $f$ can be any function that returns set of matches on input streams, we are interested in the match-functions $f$ that can be described either by a CEPL formula $\varphi$ (i.e. $f = \sem{\varphi}$) or by a MA $\cA$ (i.e. $f = \sem{\cA}$).
Let $S_1$, $S_2$ be two streams and $M_1$, $M_2$ be two matches.
We say that $S_1$ and $M_1$ are \emph{$*$-related} with $S_2$ and $M_2$, written as $(S_1,M_1)=_*(S_2,M_2)$, if $S_1[M_1] = S_2[M_2]$ (recall that $S[M]$ is the subsequence of $S$ at the positions in $M$).

Consider now any match-function $f$. We say that $f$ has the \emph{$*$-property} if, for every stream $S$ and any match $M \in f(S)$, it holds that $M' \in f(S')$ for every $S'$ and $M'$ such that $(S,M)=_*(S',M')$.
A way to understand the $*$-property is to see $S'$ as the result of fixing the tuples in $S$ that are part of the match $M$ (i.e. $S[M]$) and adding or removing tuples arbitrarily, and defining $M'$ to be the match that has the same original tuples of $M$. The following theorem states the relation that exists between the $*$-property and the $*$-semantics over MA.

\begin{proposition} \label{prop:MA_MA*}
	 If the match-function defined by a MA~$\cA$ has the $*$-property, then there exists a MA $\cA'$ such that $\sem{\cA}(S) = \ssem{\cA'}(S)$ for every $S$.
\end{proposition}
By combining Theorem~\ref{theo:CEP_MA*} and Proposition~\ref{prop:MA_MA*} we get the following useful result that shows when a match function can be defined by unary core-CEPL.
\begin{corollary}\label{cor:CEPL*}
	Let $f$ be a match function. Then $f$ can be defined by a match automaton and has the $*$-property if, and only if, there exists a formula $\varphi$ in unary core-CEPL such that $f = \sem{\varphi}$.
\end{corollary}

As it was discussed in the introduction, many query languages for CEP have been proposed in the literature and most of them include the core-CEPL fragment. 
Interestingly, the extended operators $\scand$ and $\scall$ were rather introduced in some papers since it seems that they are not strictly necessary in the core of CEPL. By using Corollary~\ref{cor:CEPL*}, we can easily understand this ``phenomena'', in the sense that $\scand$ and $\scall$ do not add expressive power to unary core-CEPL. Indeed, $\scand$ and $\scall$ can be defined by MA (Theorem~\ref{theo:extended-operators}) and both clearly satisfy the $*$-property.

\begin{corollary} \label{cor:and_all}
	For every unary CEPL formula $\varphi$ of the form $\varphi_1~\OP~\varphi_2$, with $\OP \in \{\scand, \scall\}$ and $\varphi_i$ in core-CEPL, there is a formula $\varphi'$ in unary core-CEPL such that $\sem{\varphi}(S) = \sem{\varphi'}(S)$ for every stream $S$.
\end{corollary}

Unfortunately, the $\scunless$-operator can be defined by MA but one can easily show that there exist $\scunless$-formulas which do not satisfy the $*$-property. 
Consequently, by Corollary~\ref{cor:CEPL*} this formulas cannot be defined in unary core-CEPL.
This says that $\scunless$ adds expressibility to core-CEPL and, moreover, it should be included in the design of CEP query languages that need to introduce negation.


==> in_action.tex <==
%!TEX root = ../main/main.tex

Two recurring questions in CER are what kind of patterns should users be able to express and how should a user specify these patterns. Historically, both of these questions have found their foundations in regular expressions. Unfortunately, beyond basic operations like sequencing or Kleene closure there are two some important mismatches between regular expressions and CER. First, regular expressions can only make decisions based on a local property, namely the symbol in the current position, while we expect complex events to be filtered by inspecting and correlating the data of several elements of a stream. Second, regular expressions only return boolean values, depending on whether or not a string (or, in practice, a substring) matches the regular expression. In contrast, when a CER pattern is matched, we expect to obtain not only a boolean answer, but a so-called \emph{complex event} representing the portion of the stream that was matched.\par

To overcome the aforementioned limitations, CER languages generally follow one of two approaches: they either restrict their expressive power in order to have a uniform and well-defined semantics (see for example \cite{GRUpaper, he2014}), or they include ad-hoc syntax (generally with underspecified semantics) in order to express more involved properties (e.g. \cite{SASEautomata, cayuga2, Arasu:2006}). We argue that the shortcomings of these approaches come from the fact that CER languages use first order variables, i.e., variables that bind single elements of a stream. In the rest of this section we illustrate why this makes the specification of more general properties a cumbersome process.

As a running example, suppose that sensors are positioned throughout a farm in order to detect freezing plantations. There are sensors for detecting temperature, humidity and wind speed, generating a stream of events that can have one of three types: $T$, $H$ or $W$. Suppose now that plantations might freeze if after having a temperature below 0 degrees, there is a period of fast winds in which humidity increases. In the following, we construct step by step the $\socel$ pattern that represents this situation.\par

As in most CER frameworks, \emph{filtering} is a basic operation. For example, we require to detect a temperature below 0. Languages commonly use a syntax of the form \texttt{x.temp < 0}, where \texttt{x} is the first order variable capturing the temperature event. In our framework, in contrast, variables are second order objects, and the ability to filter is expressed by arbitrary second order predicates. Following this idea, let $P_T(X)$ be the second order predicate stating that \emph{all events in $X$ must have an attribute \texttt{temp} which is less than 0}. Then, to capture temperatures below 0 degrees we write the pattern $\varphi_t=(T\cin A) \FILTER P_T(A)$. The $\scin$-operator simply pushes the captured event of type $T$ into the second order variable $A$.

Sequencing is another operation motivated by our example, specifically when we ask to see events \emph{after} a low temperature was detected. To represent sequencing we use $;$. If we have two patterns $\varphi_1$ and $\varphi_2$ then $\varphi_1;\varphi_2$ indicates that $\varphi_1$ was matched before $\varphi_2$. Therefore, our example will naturally have the form $\varphi_t; \varphi'$, where $\varphi'$ is the pattern detecting fast winds and increasing humidities. Now, this last pattern $\varphi'$ has to detect two sequences of unknown size that might occur interleaved. The fact that they might occur interleaved motivates introducing disjunction, as relevant events might belong to any of the two sequences. To specify disjunction we use the operator $\cor$. To detect sequences of unknown size we use the common Kleene closure operator $+$. Thus we will write $(W \cin B\cor H\cin C)+$ to capture the aforementioned two sequences (here $B$ and $C$ are second order variables). Now we need to filter these sequences. Let $P_W(X)$ be the second order predicate indicating that every event in $X$ represents a wind speed greater than $30$ km/h. Similarly, let $P_H(X)$ indicate that $X$ is a sequence of increasing humidity events.\par

Now we have all of the necessary ingredients to express our pattern. Define $\varphi$ as
\[\varphi := (T \cin A \FILTER \varphi_T(A))~;~(((W\cin B\cor H\cin C)+ \FILTER (P_W(B))) \FILTER (P_H(C)))\]

Using second order predicates might seem loose at first, as predicates could specify arbitrary properties. However, the goal of this approach is to separate what is inherent to a CER framework and what is particular to an application. To illustrate this, consider the language SASE introduced in \cite{SASEautomata}. Assuming that elements of type $H$ have an attribute $val$ containing the value of the humidity, to capture a sequence of increasing humidities, all above 20\%, the SASE pattern would be 
$\SEQUENCE(h\ H[]) \WHERE h[i-1].val > h[i].val \AND h.val > 20$. What is $i$? Is $h$ a first or second order variable? This pattern illustrates that introducing particular filters into a CER language often results in ad-hoc syntax with underspecified semantics. Also these ad-hoc syntax are never general. What happens if instead of an increasing sequence we want to express that the variance of the humidities is less than certain value? We do not expect the language to be capable of expressing this, but it could be a requirement for an analyst. It is also worth noting that our pattern $\varphi$ is not expressible in SASE.

According to the discussion above, we think that filtering should not be a built-in capability of CER frameworks, but that ad-hoc filtering functions should be programmed by users in a well-established programming language. And it is clear from the example that the type of objects that the users will need to create expressive filters are second order objects.


==> ucea_focel_equivalence_proof.tex <==
%!TEX root = ../main/main.tex

\subsection{Proof of Theorem~\ref{thm:equiv:socel:ucea}}

\paragraph{Construction of CEA}

Let $\cP$ be a set of unary predicates and let $\varphi$ be a formula in $\socelfull(\ext{\cP})$. We start by showing how to construct a $\ucea$ $\cA_\varphi$ over $\cP$ is equivalent to $\varphi$. Formally, this equivalence simply means that $\sem{\cA_\varphi}(S) = \sem{\varphi}(S)$ for every stream $S$. We proceed by induction, assuming that for every formula $\psi$ shorter than $\phi$ there is a $\ucea$ $\cA_\psi$ that is equivalent to $\psi$:

\begin{itemize}
	\item If $\varphi = R$, then $\cA_\varphi$ is defined as depicted in figure~\ref{fig:R_ma}, i.e. $\cA_\varphi = (\{q_1,q_2\},\Delta_\varphi,\{q_1\},\{q_2\})$ with $\Delta_\varphi = \{(q_1,\TRUE,\emptyset,q_1),(q_1,\tuples(R),\{R\},q_2)\}$
	\begin{figure}
		\begin{center}
			\begin{tikzpicture}[->,>=stealth, semithick, auto, initial text= {}, initial distance= {3mm}, accepting distance= {4mm}, node distance=4cm, semithick]
			\tikzstyle{every state}=[draw=black,text=black,inner sep=0pt, minimum size=8mm]
			\node[initial,state]	(1) 				{$q_1$};
			\node[accepting,state]	(2) [right of=1]	{$q_2$};
			\path
			(1)
			edge 				node {$\tuples(R) \mid \{R\}$} (2)
			edge [loop above] 	node {$\TRUE \mid \emptyset$} (1);
			\end{tikzpicture}
			\caption{A match automaton for $R$.}\label{fig:R_ma}
		\end{center}
	\end{figure}
	\item If $\varphi = \psi \cin A$, then $\cA_\varphi = (Q_\psi, \Delta_\varphi,I_\psi,F_\psi)$ where $\Delta_\varphi$ is the result of adding label $A$ to all non-empty transitions of $\Delta_\psi$.
	Formally, $\Delta_\varphi = \{(p,P,L,q)\in\Delta_\psi \mid L = \emptyset\}\cup\{(p,P,L,q)\mid \exists L'\neq\emptyset \text{ such that } (p,P,L',q)\in \Delta_\psi \land L=L'\cup\{L\}\}$
	
	\item If $\varphi = \pi_L(\psi)$ for some $L \subseteq \lset$, then $\cA_\varphi = (Q_\psi, \Delta_\varphi,I_\psi,F_\psi)$ where $\Delta_\varphi$ is the result of intersecting each set transition of $\Delta_\psi$ with $L$.
	Formally, that is $\Delta_\varphi = \{(p,P,L \cap L' ,q) \mid (p,P,L',q) \in \Delta_\psi\}$.
	
	\item If $\varphi = \psi \FILTER \ext{P}$ for some unary FO predicate $P$, then $\cA_\varphi = (Q_\psi, \Delta_\varphi,I_\psi,F_\psi)$ where $\Delta_\varphi$ is defined as
	$\{(p,P',L,q)\in\Delta_\psi \mid L = \emptyset\}\cup\{(p,P',L,q)\mid \exists Q \text{ such that } (p,Q,L,q)\in \Delta_\psi \land P'=Q\cap P\}$. The intuition behind this is that since $\ext(P)$ is the universal extension of $P$, all tuples that are selected must belong to $P$. \martin{please verify carefully and check it makes sense.}
	
	\item If $\varphi = \psi_1 \sq \psi_2$, then $\cA_\varphi = (Q_{\psi_1} \cup Q_{\psi_2}, \Delta_\varphi, I_{\psi_1}, F_{\psi_2})$ where $\Delta_\varphi = \Delta_{\psi_1} \cup \Delta_{\psi_2} \cup \{(p,P,L,q) \mid q \in I_{\psi_2} \land \exists q' \in F_{\psi_1}.(p,P,L,q') \in \Delta_{\psi_1}\}$.
	
	\item If $\varphi = \psi_1 \strictsq \psi_2$, then we first define the $\ucea$ $\cA_1$ (resp. $\cA_2$) so that it has the same semantics as $\cA_{\varphi_1}$ (resp. $\cA_{\varphi_2}$), but forcing it to end (resp. to begin) marking positions.
	This can be easily done by defining a new dummy state $q$ that works as final state, that is, $F_1 = \{q\}$, and for each transition that goes in a final state $q_f$ we only duplicate the transition replacing $q_f$ with $q$.
	Formally, $\cA_1 = (Q_{\psi_1} \cup \{q\}, \Delta_1, I_{\psi_1}, F_2)$, where $\Delta_1 = \Delta_{\psi_1} \cup \{(p,\alpha,L,q) \mid L \neq \emptyset \land \exists q' \in F_{\psi_1}. (p,\alpha,L,q') \in \Delta_{\psi_1} \}$.
	A similar idea can be used for $\cA_2$.
	Now, $\cA_\varphi$ is defined concatenating $\cA_1$ and $\cA_2$ in the same way as for the case of $\ssq$.
	
	\item If $\varphi = \psi \ks$, then $\cA_\varphi = (Q_\psi, \Delta_\varphi, I_\psi, F_\psi)$ where $\Delta_\varphi = \Delta_\psi \cup \{(p,P,L,q) \mid q \in I_\psi \land \exists q' \in F_\psi.(p,P,L,q') \in \Delta_\psi\}$.
	
	\item If $\varphi = \psi \strictks$, then we can mis the ideas of the cases $\ks$ and $:$. First, we add a new dummy initial state $q$ that is forced to move through marking transitions only. Then, we add a new transition $(p,P,L,q)$ for every transition $(p,P,L,q_f)$ with $q_f \in F_\psi$. Finally, the resulting automaton is $\cA_\varphi = (Q_\psi \cup \{q\}, \Delta_\varphi, I_\psi,F_\psi)$, where $\Delta_\varphi$ contains the aforementioned transitions.

	\item If $\varphi = \START(\psi)$, then we need to force the first transition to contain at least one label. To this end, we simply remove from the set of transitions of $\psi$ all transitions departing from an initial state that do not contain a label. Formally, $\cA_\varphi = (Q_\psi, \Delta_\varphi, I_\psi,F_\psi)$, where $\Delta_\varphi=\Delta_\psi\setminus\{(p,P,L,q)\mid p\in I_\psi\land L=\emptyset\}$.
	\martin{please check}.
	% we use the same technique as for $\sstrictsq$ and $\strictks$: we create a new dummy state $q$ and define $Q_\varphi = Q_\psi \cup \{q\}$, $\Delta_\varphi = \Delta_\psi \cup \{ (q,\alpha,L,q') \mid \exists p \in I_\psi. (p,\alpha,L,q') \in \Delta_\psi \land L \neq \emptyset \}$, $I_\varphi = \{q\}$ and $F_\varphi = F_\psi$.
	
	\martin{I didn't modify these, should we add some discussion}
	\item If $\varphi = \psi_1 \cor \psi_2$, then $\cA_\varphi$ is the traditional automata union between $\cA_{\psi_1}$ and $\cA_{\psi_2}$.
	
	\item If $\varphi = \psi_1 \cand \psi_2$, then $\cA_\varphi = (Q_{\psi_1} \times Q_{\psi_2}, \Delta_\varphi, I_{\psi_1} \times I_{\psi_2}, F_{\psi_1} \times F_{\psi_2})$, where $\Delta_\varphi = \{((p_1,p_2), \alpha_1 \land \alpha_2, L, (q_1,q_2)) \mid (p_i,\alpha_i,L,q_i) \in \Delta{\psi_i} \}$.
	The idea is that both automata are simulated simultaneously, forcing them to make the same marks, which results in the same match for both simulations.
	
	\item If $\varphi = \psi_1 \call \psi_2$, then we have to simulate both automata, but allowing them to end at different times.
	In order to do this, we define a new state $\bot$ so that, if an automaton is in $\bot$, it means that it has already ended and is waiting for the other automaton to accept.
	With this in mind, we define the automaton as $\cA_\varphi = (Q_\varphi, \Delta_\varphi, I_\varphi, F_\varphi)$, where $Q_\varphi = ((Q_{\psi_1} \cup \{\bot\}) \times (Q_{\psi_2} \cup \{\bot\})) \setminus \{(\bot, \bot)\}$, $I_\varphi = I_{\psi_1} \times I_{\psi_2}$, $F_\varphi = ((F_{\psi_1} \cup \{\bot\}) \times (F_{\psi_2} \cup \{\bot\})) \setminus \{(\bot,\bot)\}$ and $\Delta_\varphi = \{((p_1,p_2), \alpha_1 \land \alpha_2, L_1 \cup L_2, (q_1,q_2)) \mid (p_i,\alpha_i,L_i,q_i) \in \Delta_{\psi_i}\} \cup \{((p_1,p_2), \alpha, L, (q_1,\bot)) \mid (p_1,\alpha,L,q_1) \in \Delta_{\psi_1} \land p_2 \in F_{\psi_2} \cup \{\bot\}\} \cup \{((p_1,p_2), \alpha, L, (\bot,q_2)) \mid (p_2,\alpha,L,q_2) \in \Delta_{\psi_2} \land p_1 \in F_{\psi_1} \cup \{\bot\}\}$.
	The first part of $\Delta_\varphi$ runs both automata simultaneously, while the second and third parts simulate $\cA_{\psi_1}$ or $\cA_{\psi_2}$ alone, respectively.

	
	
	\item If $\varphi = \psi_1 \cunless \psi_2$ TODO
	
\end{itemize}

% \subsubsection{The {\texttt START} Operator}

% Here is the definition of the $\sSTART$ semantics.
% This operator falls under the class of selector operators, since it verifies a property over the match.

% Formally, the semantics of the $\sSTART$ is defined as follows.
% Given a match $M$, a stream $S$ and positions $i,j$, we say that $M \in \sem{\START(\rho)}(S,i,j)$ if $\pos(M) \neq \emptyset$, $M \in \sem{\rho}(S,i,j)$, and $\min(M) = i$.
% Intuitively, a match of $\sem{\rho}(S,i,j)$ is also in $\sem{\START(\rho)}(S,i,j)$ if it occurs at the very start of the evaluation, i.e., at position $i$.

% If $\varphi = \START(\psi)$, then the construction for $\cA_\varphi =(Q_\varphi,\Delta_\varphi,I_\varphi,F_\varphi)$ consist only on forcing the first transition to mark with at least one label.
% To accomplish this, we use the same technique as for $\sstrictsq$ and $\strictks$: we create a new dummy state $q$ and define $Q_\varphi = Q_\psi \cup \{q\}$, $\Delta_\varphi = \Delta_\psi \cup \{ (q,\alpha,L,q') \mid \exists p \in I_\psi. (p,\alpha,L,q') \in \Delta_\psi \land L \neq \emptyset \}$, $I_\varphi = \{q\}$ and $F_\varphi = F_\psi$.

\subsubsection{From CEA to unary SO-CEL}

Now we proceed to show the opposite directions. This means that given a CEA we need to define an equivalent unary SO-CEL formula. Let $\cA = (Q, \Delta, I, F)$ be a CEA, with $Q = \{q_1, \ldots, q_n\}$. Without loss of generality, assume that there is only one initial state and one final state, i.e., $I = \{q_1\}$ and $F = \{q_n\}$. Moreover, we only consider non-zero executions, that is, an accepting run of a CEA must be of length at least $1$. Notice that this limits automata to not being able to run over the empty stream, but since we only care about large (potentially infinite) streams, this case is not of interest.

In the sequel we define a formula $\varphi_\cA$ such that $\sem{\cA}(S) = \sem{\varphi_\cA}(S)$ for every $S$. The main idea is based on the traditional construction from DFA which defines, for every pair of states $q_i, q_j$, a CEPL formula $\varphi_{ij}$ that represents the complex events defined by the runs from $q_i$ to $q_j$. Furthermore, we define $\varphi_{ij}^k$ the same way but with the restriction that the runs only pass through states $q_1, \ldots, q_k$.
It is clear that $\varphi_{ij}^{|Q|} = \varphi_{ij}$.

To simplify the construction, we give some definitions.
First, we define the $\FALSE$ formula as a formula that is never satisfied.
One way to define it is $\FALSE = (R \as x \FILTER \FALSE)$, but we will use $\FALSE$ to keep the proof simple.
Also, if $\alpha$ is a formula and $R$ is a relation, we define $\alpha[R]$ as the formula that results after replacing in $\alpha$ every occurrence of $\type(x)=R$ with $\TRUE$ and every occurrence of $\type(x)=R'$ with $\FALSE$ for all $R' \neq R$.

Now we define $\varphi_{ij}^k$ recursively in the following way.
The base case $k = 0$ is defined as:
\[
\varphi_{ij}^0 = \left\{
\renewcommand{\arraystretch}{1.3}
\begin{array}{ll}
\rho^\alpha_L & \text{if $(q_i,\alpha, L,q_j) \in \Delta$ for some $\alpha$ and $L$}\\
\FALSE & \text{otherwise}
\end{array}
\right.
\]
where $\rho^\alpha_L$ represents the CEPL formula that accepts all matches with a single event that satisfies $\alpha$ and assigns the labels $L$.
We define this formula as $\rho^\alpha_L := ( \ldots (\rho_\alpha \cin A_1) \ldots ) \cin A_l$, where $L = \{A_1, \ldots, A_l\}$ and $\rho_\alpha = R_1 \FILTER \alpha[R_1] \cor \cdots \cor R_r \FILTER \alpha[R_r]$ for $\cR = \{R_1, \ldots, R_r\}$.

Next, the recursion is defined as:
\begin{equation}
\varphi_{ij}^k \; = \; \varphi_{ij}^{k-1} \cor (\varphi_{ik}^{k-1} \strictsq \varphi_{kj}^{k-1}) \cor (\varphi_{ik}^{k-1} \strictsq \varphi_{kk}^{k-1}\ks \strictsq \varphi_{kj}^{k-1}) \label{eq:formula}
\end{equation}
Finally, the final formula $\varphi_\cA$ is the result of considering $\varphi_{1n}$ and projecting to retrieve only the labels of $\cA$.
Formally, we define it as $\varphi_\cA := \pi_L( \START( \varphi_{1n} ) ) $, where $L$ is the set of labels in $\cA$.
The $\START$ only forces the match to begin immediately at position $0$, and the projection is needed so that the result does not contain the default labels assigned by the formula.
We assume that $L \cap \cR = \emptyset$, therefore no label is mistakenly projected.

Now, we will prove that the construction satisfies the theorem, i.e., $\sem{\cA}(S) = \sem{\varphi_\cA}(S)$ for every stream $S$.


\subsection{Proof of Lemma~\ref{lem:strict-contained-in-contiguous}}

\begin{proof}
	Consider a formula $\varphi$ in $\text{core-CEPL} \cup \{\STRICT\}$.
	We first prove that for every formula $\varphi'$ in $\text{core-CEPL} \cup \{\STRICT\}$ there is a formula $\psi'$ in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$ that is equivalent to $\STRICT(\varphi')$, for which we do induction over the length of $\varphi'$.
	The base case is $\varphi' = R \as x$, which clearly satisfies the above considering $\psi' = R \as x$.
	For the inductive step, consider the following cases.
	\begin{itemize}
		\item If $\varphi' = \rho_1 \sq \rho_2$, then $\STRICT(\varphi') \equiv \STRICT(\rho_1) \strictsq \STRICT(\rho_2)$.
		By induction hypothesis, both $\STRICT(\rho_1)$ and $\STRICT(\rho_2)$ have equivalent formulas $\sigma_1$ and $\sigma_2$, respectively, in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$.
		Thus, $\psi' = \sigma_1 \strictsq \sigma_2$ is equivalent to $\STRICT(\varphi')$.
		\item If $\varphi' = \rho \FILTER \alpha$, then $\STRICT(\varphi') \equiv \STRICT(\rho) \FILTER \alpha$.
		By induction hypothesis, $\STRICT(\rho)$ has an equivalent formula $\sigma$ in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$.
		Thus, $\psi' = \sigma \FILTER \alpha$ is equivalent to $\STRICT(\varphi')$.
		\item If $\varphi' = \rho_1 \cor \rho_2$, then $\STRICT(\varphi') \equiv \STRICT(\rho_1) \cor \STRICT(\rho_2)$.
		By induction hypothesis, both $\STRICT(\rho_1)$ and $\STRICT(\rho_2)$ have equivalent formulas $\sigma_1$ and $\sigma_2$, respectively, in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$.
		Thus, $\psi' = \sigma_1 \cor \sigma_2$ is equivalent to $\STRICT(\varphi')$.
		\item If $\varphi' = \rho \ks$, then $\STRICT(\varphi') \equiv \STRICT(\rho) \strictks$.
		By induction hypothesis, $\STRICT(\rho)$ has an equivalent formula $\sigma$ in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$.
		Thus, $\psi' = \sigma \strictks$ is equivalent to $\STRICT(\varphi')$.
	\end{itemize}
	After this the only thing left is to replace every subformula $\varphi'$ of $\varphi$ with its equivalent $\psi'$, and the resulting formula will be in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$ and will be equivalent to $\varphi$, thus proving the lemma.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:contiguous-sequence-contained-strict}}

\begin{proof}
	Consider a formula $\varphi$ in $\text{core-CEPL} \cup \{\strictsq\}$.
	We first prove that for every formula $\varphi' = \varphi_1 \strictsq \varphi_2$ with $\varphi_1$ and $\varphi_2$ in $\text{core-CEPL} \cup \{\STRICT\}$ there exists a formula $\psi'$ equivalent to $\varphi'$ in $\text{core-CEPL} \cup \{\STRICT\}$.
	We prove this by doing induction over the length of $\varphi'$.
	The base case is $\varphi' = R \as x \strictsq T \as y$ for some $R$, $T$, $x$ and $y$.
	Clearly $\varphi'$ is equal to $\psi' = \STRICT(R \as x \sq T \as y)$.
	For the inductive step consider the following cases:
	\begin{itemize}
		\item If $\varphi_1 = \rho_1 \sq \rho_2$, then $\varphi' \equiv \rho_1 \sq (\rho_2 \strictsq \varphi_2)$.
		By induction hypothesis, $(\rho_2 \strictsq \varphi_2)$ has an equivalent formula $\sigma$ in $\text{core-CEPL} \cup \{\STRICT\}$.
		Thus, $\psi' = \rho_1 \sq \sigma$ is equivalent to $\varphi'$.
		\item If $\varphi_1 = \rho \FILTER \alpha$, then $\varphi' \equiv (\rho \strictsq \varphi_2) \FILTER \alpha$.
		By induction hypothesis, $(\rho \strictsq \varphi_2)$ has an equivalent formula $\sigma$ in $\text{core-CEPL} \cup \{\STRICT\}$.
		Thus, $\psi' = \sigma \FILTER \alpha$ is equivalent to $\varphi'$.
		\item If $\varphi_1 = \rho_1 \cor \rho_2$, then $\varphi' \equiv (\rho_1 \strictsq \varphi_2) \cor (\rho_2 \strictsq \varphi_2)$.
		By induction hypothesis, both $(\rho_1 \strictsq \varphi_2)$ and $(\rho_2 \strictsq \varphi_2)$ have equivalent formulas $\sigma_1$ and $\sigma_2$, respectively, in $\text{core-CEPL} \cup \{\STRICT\}$.
		Thus, $\psi' = \sigma_1 \cor \sigma_2$ is equivalent to $\varphi'$.
		\item If $\varphi_1 = \rho \ks$, then $\varphi' \equiv (\rho \strictsq \varphi_2) \cor (\rho \ks \sq (\rho \strictsq \varphi_2))$.
		By induction hypothesis, $(\rho \strictsq \varphi_2)$ has an equivalent formula $\sigma$ in $\text{core-CEPL} \cup \{\STRICT\}$.
		Thus, $\psi' = \sigma \cor (\rho \ks \sq \sigma)$ is equivalent to $\varphi'$.
	\end{itemize}
	The cases regarding the structure of $\varphi_2$ instead of $\varphi_1$ are analogous to the previous ones.
	
	Then, every subformula $\varphi'$ of $\varphi$ is replaced by its equivalent $\psi'$ in a bottom-up fashion to ensure that the subformulas of $\varphi'$ are indeed in $\text{core-CEPL} \cup \{\STRICT\}$.
	Finally, the resulting formula $\psi$ is clearly in $\text{core-CEPL} \cup \{\STRICT\}$ and is equivalent to $\varphi$.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:strict-unary-equivalence}}

\begin{proof}
	Consider a unary formula $\varphi$ in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$.
	We first prove that there is a formula $\psi$ in $\text{core-CEPL} \cup \{\strictsq, \STRICT\}$ which is equivalent to $\varphi$, and then the proof follows directly by the previous lemma.
	
	Consider any unary formula $\varphi'$ in $\text{core-CEPL} \cup \{\strictsq, \STRICT\}$.
	We prove by induction that there exists a formula $\psi'$ in $\text{core-CEPL} \cup \{\strictsq, \STRICT\}$ which is equivalent to $\varphi' \strictks$.
	Assume w.l.o.g. that $\varphi'$ is in LP-normal form and, moreover, in disjunctive-normal form.
	Now, consider the following cases:
	\begin{itemize}
		\item For the base case, if $\varphi' = R \as x$, then $\psi' = \STRICT(R \as x \ks)$ is equivalent to $\varphi' \strictks$.
		Similarly, if $\varphi' = R \as x \FILTER \alpha$, then $\psi' = \STRICT(R \as x \FILTER \alpha \ks)$.
		\item If $\varphi' = \STRICT(\varphi_1)$, then $\psi' = \STRICT(\varphi_1 \ks)$ is equivalent to $\varphi' \strictks$.
		\item If $\varphi' = \varphi_1 \sq \varphi_2$, then $\psi' = \varphi_1 \sq (\varphi_2 \cor ((\varphi_2 \strictsq \varphi_1) \ks \sq \varphi_2))$ is equivalent to $\varphi' \strictks$.
		\item If $\varphi' = \varphi_1 \ks$, then $\psi' = \varphi_1 \ks$ is equivalent to $\varphi' \strictks$.
	\end{itemize}
	
	The last and more complex operator is the $\scor$, for which we have to consider all possible cases for $\varphi_1$ and $\varphi_2$.
	The simplest scenario is where both $\varphi_1$ and $\varphi_2$ have either the form $R \as x$, $R \as x \FILTER \alpha$ or $\STRICT(\psi)$ for some $\psi$, at which case we can simply write $\varphi'\strictks$ as $\STRICT(\varphi' \ks)$.
	Notice that, since $\varphi'$ is said to be in LP-normal form, then the only occurrences of $\FILTER$ could be of this form.
	
	Now we consider the cases where some of them does not have this form (w.l.o.g. assume is $\varphi_2$).
	Moreover, since $\varphi'$ is in disjunctive-normal form, we assume that all the remaining $\scor$'s are in the side of $\varphi_1$, therefore do not consider the $\scor$-case for $\varphi_2$.
	Now, consider the case $\varphi_2 = \rho_1 \sq \rho_2$.
	Here we use the following equivalence:
	
	\[
	\begin{array}{rcll}
	(\varphi_1 \cor (\rho_1 \sq \rho_2)) \strictks &\equiv& \varphi_1 \strictks \cor (\rho_1 \sq \rho_2) \strictks \cor&(1)\\ 
	&&(\varphi_1 \strictks \strictsq (\rho_1 \sq \rho_2) \strictks) \strictks \cor & (2)\\
	&&\varphi_1 \strictks \strictsq ((\rho_1 \sq \rho_2) \strictks \strictsq \varphi_1 \strictks) \strictks \cor & (3)\\
	&&((\rho_1 \sq \rho_2)\strictks \strictsq \varphi_1 \strictks)\strictks \cor& (4)\\
	&&(\rho_1 \sq \rho_2)\strictks \strictsq (\varphi_1 \strictks \strictsq (\rho_1 \sq \rho_2))\strictks& (5)
	\end{array}
	\]
	Here, part $(1)$ has no problem since the $\strictks$-operator is applied over subformulas of the original one, thus by induction hypothesis they can be written without $\strictks$.
	Moreover, with some basic transformations in part $(2)$ (replacing $(\rho_1 \sq \rho_2)\strictks$ by $\rho_1 \sq (\rho_2 \cor ((\rho_2 \strictsq \rho_1)\ks \sq \rho_2))$) one can show that it is equivalent to the formula $(\sigma_1 \sq \sigma_2) \strictks$, where $\sigma_1 = \varphi_1 \strictks \strictsq \rho_1$ and $\sigma_2 = \rho_2 \cor ((\rho_2 \strictsq \rho_1) \ks \sq \rho_2)$.
	Then, we can replace $(\sigma_1 \sq \sigma_2)$ with $\sigma_1 \sq (\sigma_2 \cor ((\sigma_2 \strictsq \sigma_1)\ks \sq \sigma_2))$, and the resulting formula will contain only one $\strictks$ in the form $\varphi_1 \strictks$, which by induction hypothesis can also be removed.
	Similarly, parts $(3)$, $(4)$ and $(5)$ can be rewritten this way, therefore for the case of $\varphi_2 = \rho_1 \sq \rho_2$ the induction statement remains true.
	
	Now consider the case $\varphi_2 = \rho\ks$.
	Notice that, by expanding the definition of the $\ks$-operator ($\rho \ks \equiv \rho \cor \rho \sq \rho \ks$), $\varphi'$ can then be written as $(\varphi_1 \cor \rho) \cor (\rho \sq \rho \ks)$.
	Then, if we redefine $\varphi_1 := (\varphi_1 \cor \rho)$ and $\varphi_2 ;= (\rho \sq \rho \ks)$, clearly $\varphi'$ would have the form $\varphi_1 \cor (\rho_1 \sq \rho_2)$.
	Therefore, we can apply the previous case and the resulting formula will still satisfy the induction statement, thus it remains true in the case $\varphi_2 = \rho \ks$.
	
	Then, we can replace every subformula $\varphi'$ of $\varphi$ with its equivalent $\psi'$ in a bottom-up fashion to ensure that the subformulas of $\varphi'$ satisfy the condition of being in $\text{core-CEPL} \cup \{\strictsq, \STRICT\}$.
	Finally, the remaining formula $\psi$ does not contain $\strictks$ and thus is in $\text{core-CEPL} \cup \{\strictsq, \STRICT\}$.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:strict-proper-containment}}

\begin{proof}
	We show that for the formula $\varphi = (A \as x \sq E \as y \FILTER x.a = y.a)\strictks$ in $\text{core-CEPL} \cup \{\strictsq, \strictks\}$ there is no equivalent formula $\psi$ in $\text{core-CEPL} \cup \{\STRICT\}$.
	For this we first give a few somehow useful definitions.
	
	Consider a stream $S$, a match $M$, a valuation $\nu$, two positions $i,j \in M$ with $i < j$ and a constant $k \geq 1$.
	Then, the result of pumping the fragment $[i,j]$ of $(S,M,\nu)$ $k$ times is a triple $(S',M',\nu')$ where $S'$, $M'$ and $\nu'$ are a stream, match and valuation, respectively, defined as follows.
	Consider the factorization $M_1 \cdot M_2 \cdot M_3$ of $M$, where $M_1$ contains all positions in $M$ that are lower than $i$, $M_2$ contains all positions of $M$ between $i$ and $j$ (including them) and $M_3$ contains all positions of $M$ higher than $j$.
	Likewise, consider the factorization $S_1 \cdot S_2 \cdot S_3$ of $S$ in the same way and, moreover, let $\nu_1$, $\nu_2$ and $\nu_3$ be a ``partition'' of the valuation $\nu$ in a way that $\nu_i$ only assign the variables of the section $M_i$, i.e., $\nu_i(x) = \nu(x)$ iff $\nu(x) \in M_i$.
	Now, if $M_2$ is not a contiguous interval (that is, if there is some $l$ such that $i < l < j$ and $l \notin M_2$), then define $S'$ as $S_1 \cdot P_0 \cdot S_2 \cdot P_1 \cdot S_2 \cdot \ldots \cdot S_2 \cdot P_k \cdot S_3$, where $S_2$ is repeated $k$ times and each $P_i$ is an arbitrary finite stream.
	On the other hand, if $M_2$ is a contiguous interval, define $S'$ the same way but without the $P_i$, i.e., $S' = S_1 \cdot S_2 \cdot S_2 \cdot \ldots \cdot S_2 \cdot S_3$.
	Similarly, define $M'$ as $M_1 \cdot M_2^1 \cdot M_2^2 \cdot \ldots \cdot M_2^k \cdot M_3'$, where each $M_2^i$ is the same match $M_2$ but with its positions moved to fit the $i$-th occurrence of $S_2$ in $S'$.
	For example, $M_2^2$ results after adding $|S_2|$ to all positions of $M_2$ if it is a contiguous interval, and adding $|P_0| + |S_2| + |P_1|$ else.
	$M_3'$ is the same as $M_3$ but moved to fit $S_3$.
	Notice that if $M$ is a contiguous interval, then $M'$ also is.
	Moreover, let $\nu_1'$, $\nu_2'$ and $\nu_3'$ be the valuations such that $\nu_i'$ is the same as $\nu_i$ but with its positions moved to fit the corresponding events in the part $S_i$ of $S'$.
	Then, define the valuation $\nu'$ as $\nu_1'[\nu_2' \rightarrow \dom(\nu_2')][\nu_3' \rightarrow \dom(\nu_3')]$, this is, the result of merging valuations $\nu_1'$, $\nu_2'$ and $\nu_3'$ together into one.
	Notice that $\nu'$ points at the same events in $S'$ as $\nu$ does in $S$, thus $\nu'_{S'}(x) = \nu_S(x)$ for every $x$.
	
	A formula $\rho$ in CEPL is said to be \textit{pumpable} if there exists a constant $N \in \bbN$ such that for every stream $S$, valuation $\nu$, position $p$ and match $M \in \sem{\rho}(S,p,\nu)$ with $|M| > N$ there exist two positions $i,j \in M$ with $i < j$ such that for every $k \geq 1$ it holds that $M' \in \sem{\rho}(S',p,\nu')$, where $(S',M',\nu')$ is the results of pumping the fragment $[i,j]$ of $(S,M,\nu)$ $k$ times.
	In the following lemma we show the utility of this property.
	
	\begin{lemma}
		Every formula $\varphi$ in $\text{core-CEPL} \cup \{\STRICT\}$ is pumpable.
	\end{lemma}
	\begin{proof}
		Consider a formula $\varphi$ in $\text{core-CEPL} \cup \{\STRICT\}$.
		We prove the lemma by induction over the length of $\varphi$.
		First, consider the base case $R \as x$.
		Then, by defining $N = 1$ we know that for every stream $S$ there is no match $M \in \sem{\varphi}(S)$ with $|M| > N$, so the lemma holds.
		
		Now, for the inductive step consider first the case $\varphi = \psi_1 \FILTER \alpha$.
		By induction hypothesis, we know that the lemma holds for $\psi_1$, thus let $N_1$ be its corresponding constant.
		Let $N$ be equal to $N_1$.
		Consider any stream $S$, valuation $\nu$, position $p$ and match $M \in \sem{\varphi}(S, p, \nu)$ with $|M| > N$.
		By definition $M \in \sem{\psi_1}(S, p, \nu)$ and $\nu_S \models \alpha$.
		By induction hypothesis, $\psi_1$ is pumpable, thus there exist positions $i,j \in M$ with $i < j$ such that the fragment $[i,j]$ can be pumped.
		Moreover, consider that the result of pumping the fragment $[i,j]$  $k$ times is $(S',M',\nu')$, for an arbitrary $k$.
		Then, it holds that $M' \in \sem{\psi_1}(S',\nu',p)$.
		Also, because in the pumping it holds that $\nu_S(x) = \nu'_{S'}(x)$ for every $x$, then $\nu'_{S'} \models \alpha$.
		Therefore, $M' \in \sem{\varphi}(S',\nu',p)$, thus $\varphi$ is pumpable.
		
		Consider now the case $\varphi = \psi_1 \cor \psi_2$.
		By induction hypothesis, we know that the lemma holds for $\psi_1$ and $\psi_2$, thus let $N_1$ and $N_2$ be the corresponding constants, respectively.
		Then, we define the constant $N$ as the maximum between $N_1$ and $N_2$.
		Consider any stream $S$, valuation $\nu$, position $p$ and match $M \in \sem{\varphi}(S,p,\nu)$ with $|M| > N$.
		Either $M \in \sem{\psi_1}(S,p,\nu)$ or $M \in \sem{\psi_2}(S,p,\nu)$, so w.l.o.g. consider the former case.
		By induction hypothesis, $\psi_1$ is pumpable, thus there exist positions $i,j \in M$ with $i < j$ such that the fragment $[i,j]$ can be pumped and the result $(M',S',\nu')$ satisfies $M' \in \sem{\psi_1}(S',p,\nu')$.
		This means that $M' \in \sem{\varphi}(S',p,\nu')$, therefore, $\varphi$ is pumpable.
		
		Now, consider the case $\varphi = \psi_1 \sq \psi_2$.
		By induction hypothesis, we know that the lemma holds for $\psi_1$ and $\psi_2$, thus let $N_1$ and $N_2$ be the corresponding constants, respectively.
		Then, we define the constant $N = N_1 + N_2$.
		Consider any stream $S$, valuation $\nu$, position $p$ and match $M \in \sem{\varphi}(S,p,\nu)$ with $|M| > N$.
		This means that there exist matches $M_1$ and $M_2$ with $M = M_1 \cdot M_2$ such that $M_1 \in \sem{\psi_1}(S,p,\nu)$ and $M_2 \in \sem{\psi_2}(S,j,\nu)$, where $j = \max(M_1) + 1$.
		Moreover, either $|M_1| > N_1$ or $|M_2| > N_2$, so w.l.o.g. assume the former case.
		By induction hypothesis, $\psi_1$ is pumpable, thus there exist positions $i,j \in M$ with $i < j$ such that the fragment $[i,j]$ can be pumped and the result $(M_1',S',\nu')$ satisfies $M_1' \in \sem{\psi_1}(S',p,\nu')$.
		Assume that the pumping added $r$ new events, and define the match $M' = M_1' \cdot M_2'$, where $M_2'$ is the same as $M_2$ but adding $r$ to each position (so that the events of $S'[M_2']$ are the same as $S[M_2]$).
		Then $M_1' \in \sem{\psi_1}(S',p,\nu')$ and $M_2' \in \sem{\psi_2}(S,j+r,\nu')$, thus $M' \in \sem{\varphi}(S')$, therefore, $\varphi$ is pumpable.
		
		Consider then the case $\varphi = \psi_1 \ks$.
		By induction hypothesis, we know that the lemma holds for $\psi_1$, thus let $N_1$ be its corresponding constant.
		Let the constant $N$ be equal to $N_1$.
		Consider any stream $S$, valuation $\nu$, position $p$ and match $M \in \sem{\varphi}(S,p,\nu)$ with $|M| > N$.
		Then, consider $i = \min(M)$ and $j = \max(M)$, consider any $k \geq 1$ and let $(S',M',\nu')$ be the result of pumping the fragment $[i,j]$ of $(S,M,\nu)$ $k$ times.
		We prove now that $M' \in \sem{\varphi}(S',p,\nu')$ by induction over $k$.
		If $k = 1$ then, as defined in the definition of pumping, $S'$ has the form $S_1 \cdot P_0 \cdot S_2 \cdot P_1 \cdot S_3$, and $M'$ is the same as $M$ but adding $r$ to each position, where $r = |P_0|$.
		Clearly it holds that $M' \in \sem{\varphi}(S',p,\nu')$, since the modifications did not affect the matching part of $S$.
		Now, consider that $k > 1$.
		Then, $S'$ has the form $S_1 \cdot P_0 \cdot S_2 \cdot P_1 \cdot S_2 \cdot \ldots \cdot S_2 \cdot P_k \cdot S_3$.
		Similarly, $M'$ is defined as $M_1 \cdot M_2^1 \cdot M_2^2 \cdot \ldots \cdot M_2^k \cdot M_3'$, where $M_1 = M'_3 = \emptyset$ and each $M_2^i$ is the same match $M$ but with its positions moved to fit the $i$-th occurrence of $S_2$ in $S'$.
		Consider that $r = |S_1 \cdot P_0 \cdot S_2|$.
		By induction hypothesis, we can say that $M_2' \in \sem{\varphi}(S',r+1,\nu')$ where $M_2' = M_2^2 \cdot \ldots \cdot M_2^k$ (notice that we consider it from position $r+1$ because there is no lower position in the match).
		Also, it is easy to see that this implies $M_2' \in \sem{\varphi \ks}(S',r,\nu')$, which is something we will need next.
		Moreover, it holds that $M_2^1 \in \sem{\varphi}(S',p,\nu')$, because it represents the same match as the original one $M$.
		Notice that here the valuation $\nu'$ does not affect because it is overwritten by another one after evaluating inside the $\ks$-operator.
		Then, because $M' = M_2^1 \cdot M_2'$, it follows that $M' \in \sem{\varphi \sq \varphi \ks}(S',p,\nu')$ which also implies that $M' \in \sem{\varphi \ks}(S',p,\nu')$.
		Since $\varphi \ks = \psi_1 \ks \ks \equiv \psi_1 \ks = \varphi$, it holds that $M' \in \sem{\varphi}(S',p,\nu')$.
		
		Finally, consider the case $\varphi = \STRICT(\psi_1)$.
		By induction hypothesis, we know that the lemma holds for $\psi_1$, thus let $N_1$ be its corresponding constant.
		Let the constant $N$ be equal to $N_1$.
		Consider any stream $S$, valuation $\nu$, position $p$ and match $M \in \sem{\varphi}(S,p,\nu)$ with $|M| > N$.
		Then, by definition $M \in \sem{\psi_1}(S,p,\nu)$, and by induction hypothesis there exist positions $i,j \in M$ such that the fragment $[i,j]$ can be pumped and the result $(M',S',\nu')$ satisfies $M' \in \sem{\psi_1}(S,p,\nu')$.
		Notice that $M$ is a contiguous interval because of the definition of $\STRICT$, therefore $M'$ is also a contiguous interval, thus $M' \in \sem{\varphi}(S,p,\nu')$.
	\end{proof}
	
	Now, we show that there is no formula $\psi$ in $\text{core-CEPL} \cup \{\STRICT\}$ equivalent to $\varphi$ by proving that such formula is not pumpable.
	By contradiction, assume that $\psi$ exists, and let $N$ be its constant.
	Consider then the stream:
	\[
	S = \begin{array}{cccc}
	\begin{array}{cccccc}
	A & L & E & A & L & E \\
	1 & 1 & 1 & 2 & 2 & 2
	\end{array} & \cdots & \begin{array}{ccc}
	A & L & E \\
	N & N & N
	\end{array} & \cdots
	\end{array}
	\]
	Where the first and second lines are the type and $a$ attribute of each event, respectively, and consider the match $M = \{1, 3, 4, 6, \ldots , 3 \cdot N\}$.
	Now, let $i,j \in M$ be any two positions of the match, which define the partition $M_1 \cdot M_2 \cdot M_3$, and name $t_1 = S[i]$ and $t_2 = S[j]$.
	We will use $k = 2$, i.e., repeat section $S[i,j]$ two times, and use the 1-tuple stream $U(0)$ as the arbitrary streams $P_0$ and $P_1$ to get the resulting stream $S'$ and the corresponding match $M'$ and valuation.
	We will analyse the following possible cases: $\type(t_1) = \type(t_2)$; $\type(t_1) = A$ and $\type(t_2) = E$; $\type(t_1) = E$ and $\type(t_2) = A$.
	In the first case the resulting $M'$ is a match with two consecutive tuples of the same type, which contradicts the original formula $\varphi$.
	In the second case $M_2$ is not a contiguous interval so the match $M'$ would fail to ensure that the $A$ tuple following $t_2$ is placed right after it (because of the tuple $U(0)$ between), thus contradicting the $\strictks$ property of $\varphi$.
	In the third case it is clear that the last $A$ in the first repetition of $[i,j]$ and the first $E$ in the second repetition (i.e., $S[j]$ and $S[j+2]$) do not satisfy the $\sFILTER$ condition because $S[j].a > S[j+2].a$.
	Finally, the formula $\psi$ cannot exist.
\end{proof}



==> unary_expr_old.tex <==
%!TEX root = ../main/main.tex



\subsection{Complex Event Automata}\label{subsec:ma}

\stijn{Shouldn't we call this Unary Complex Event Automata ?}
To study the computational power of core formulas, we extend the automata model introduced in~\cite{GRUpaper}, called \emph{match automata}, in order to handle correctly complex events and not only matches (i.e. sets of positions).
Given $t \in \tuples(\cR)$ and a unary predicate $\alpha$ in FO logic, we say that $t$ satisfies $\alpha$, denoted by $t \models \alpha$, if $\sigma_t \vDash \alpha$ where $\sigma_t$ is the function that assigns $t$ to every variable in $\alpha$ (i.e. $\sigma_t(x) = t$ for every variable $x$ in $\alpha$).
Given a schema $\cR$, let $\fset_u(\cR)$ be the set of formulas that contains all (FO) unary predicates and is closed under $\land$ and $\lor$.\martin{same here, first order should be closed under negation}

Let $\cR$ be a schema and $\lset$ a set of labels such that $\cR \subseteq \lset$.
A \emph{complex event automaton} (CEA) over $\cR$ is a tuple $\cA = (Q, \Delta, I, F)$ where $Q$ is a finite set of states, $\Delta \subseteq Q \times \fset_u(\cR) \times 2^\lset \times Q$ is a finite transition relation, and $I, F \subseteq Q$ are the set of initial and final states, respectively.
Given an $\cR$-stream $S = t_0 t_1 \ldots$, a run $\rho$ of length $n$
of $\cA$ over $S$ is a sequence of transitions:
$\rho: q_0 \ \trans{\alpha_0 / L_0} \ q_1 \  \trans{\alpha_1 / L_1} \ \cdots \ \trans{\alpha_n / L_n} \ q_{n+1}$
such that $q_0 \in I$, $t_i \vDash \alpha_i$ and $(q_i, \alpha_{i}, L_{i}, q_{i+1}) \in \Delta$ for every $i \leq n$.
We say that $\rho$ is \emph{accepting} if $q_{n+1} \in F$, and denote by $\run_n(\cA, S)$ the set of accepting runs of $\cA$ over $S$ of length $n$.
Further, we define the complex event $C_\rho:\lset \rightharpoonup 2^\bbN$  induced by $\rho$ as $C_\rho(A) = \{i \in [0,n] \mid A \in L_i\}$.
Given a stream $S$ and $n \in \bbN$, we define the set of complex events of $\cA$ over $S$ at position $n$ as $\sem{\cA}_n(S) = \{C_\rho \mid \rho \in \run_n(\cA, S) \}$ and the set of all complex events as $\sem{\cA}(S) = \bigcup_n \sem{\cA}_n(S)$.

It is important to note that our definition of complex event automaton
differs from the definition of match automaton in two aspects. First, in CEA we mark the events using labels of $\lset$, unlike in \cite{GRUpaper}, where an event is either marked or unmarked by using the symbols $\amark$ or $\umark$, respectively.
The empty set $\emptyset$ in the new model is the analog of $\umark$-symbol meaning that no label is assign to the position. On the other hand, a non-empty set $L \subseteq \lset$ marks a position with a set of labeled providing more structure and context to the former output.
Second, complex event automata do not require a marking transition at the end of every accepting run, in contrast to match automata. 
This relaxation helps to increase the expressibility of the computational model with the cost of loosing some closure properties as we showed below.
For these two difference, we called this new model complex event automaton instead of match automaton.  

We say that a complex event automaton $\cA$ is I/O-deterministic (i.e. Input/Output deterministic) if $|I| = 1$ and for any two transitions $(p,\alpha_1,L_1,q_1)$ and $(p,\alpha_2,L_2,q_2)$, if  $L_1 = L_2$ then $\alpha_1$ and $\alpha_2$ are mutually exclusive (i.e. for every $t$ it is not true that $t \models \alpha_1$ and $t \models \alpha_2$). 
Notice that an I/O-deterministic CEA behaves deterministically when the stream and complex event are given. 
We say that CEA are closed under I/O-determinization (complement) if for every CEA $\cA$, there exists a I/O-deterministic CEA $\cA^{\text{det}}$ (a CEA $\cA^\text{c}$ resp.) such that for every stream $S$ we have $\sem{\cA^{\text{det}}}(S) = \sem{\cA}(S)$ ($\sem{\cA^\text{c}}(S) = \{C: \lset \rightharpoonup 2^\bbN \mid \text{$C$ is finite}\} \setminus \sem{\cA}(S)$ resp.).
Furthermore, we say that $\cA$ is closed under union (intersection) if
for every CEA $\cA_1$ and $\cA_2$, there exists a CEA $\cA$ such that
for every stream $S$ we have $\sem{\cA}(S) = \sem{\cA_1}(S) \cup
\sem{\cA_2}(S)$ ($\sem{\cA}(S) = \sem{\cA_1}(S) \cap \sem{\cA_2}(S)$
resp.).

\stijn{Don't we have closure in the stricter sense where $\sem{\cA}_n(S) = \sem{\cA_1}_n(S) \cup
\sem{\cA_2}_n(S)$ ($\sem{\cA}_n(S) = \sem{\cA_1}_n(S) \cap
\sem{\cA_2}_n(S)$) ?? This closure implies the proposition below, but
the converse is not necessarily true (I think)}

\begin{proposition} \label{prop:CEA_closure}
	CEA are closed under union, intersection, and I/O-determinization, but not under complement.
\end{proposition}

To see why CEA are not closed under complement consider the example in Figure~\ref{fig:complement_CEA}. 
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[->,>=stealth, semithick, auto, initial text= {}, initial distance= {3mm}, accepting distance= {4mm}, node distance=2.5cm, semithick]
		\tikzstyle{every state}=[draw=black,text=black,inner sep=0pt, minimum size=8mm]
		\node[initial,state]	(1) 				{$q_1$};
		\node[state]			(2) [right of=1]	{$q_2$};
		\node[accepting,state]	(3) [right of=2]	{$q_3$};
		\path
		(1)
		edge 				node {$\alpha(x) \mid M$} (2)
		edge [loop above] 	node {$\TRUE \mid \emptyset$} (1)
		(2)
		edge [loop above] node {$\TRUE \mid \emptyset$} (2)
		edge node {$\beta(x) \mid \emptyset$} (3);
		\end{tikzpicture}
		\vspace{-.1cm}
		\caption{A complex event automaton whose complement cannot be defined by a CEA. Here $\alpha(x) := \type(x)=H$ and $\beta(x) := \type(x)=T$.}\label{fig:complement_CEA}
		\vspace{-.3cm}
	\end{center}
\end{figure}
Intuitively, this automaton marked an $H$-event with $M$ if there exists some $T$-event afterwards. Then its complement would have to marked all $H$-event where there exists no $T$-event in the future which, of course, it is impossible to checked by a complex event automaton. 

In~\cite{GRUpaper}, it was shown that every match automaton can be evaluated efficiently over a data stream with linear time per data-item and constant-delay enumeration of matches. This is one of the corner-stone to have an efficient evaluation of CEP formulas with unary filters. Therefore, it is natural to ask whether the new model of CEA can also be evaluated efficiently. As one could expect, by slightly modifying the algorithmic techniques introduced in~\cite{GRUpaper}, we can evaluate every CEA efficiently over a data stream with linear time per data-item and constant-delay enumeration.

\begin{proposition} \label{prop:evaluation}
	Every CEA can be evaluated efficiently over a data stream with linear time per data-item and constant-delay enumeration.
\end{proposition}

\subsection{Expressiveness of Unary Core Formulas}\label{subsec:expressiveness}

As it was shown in Section~\ref{sec:comparison}, core formulas with SO-variables coincide with FO-variables when we restrict to unary filters. 
Furthermore, it was shown in~\cite{GRUpaper} that every unary core formula with FO-variables can be computed by a match automaton.
\stijn{I guess what we means in the following section is that for
  every set of unary first order predicates $P$, we have that for
  every formula in $SO-CEL(P^e)$ there exists a CEA using predicates
  in $P$ that computes the same set of complex events. Note that this
  need not be true if the SO-CEL formula uses arbitrary unary SO
  predicates that are not extension of FO predicates.}
Actually, one can easily see that the same will hold for unary core formulas with SO-variables and complex event automata: for every unary core formula with SO-variable there exists an CEA that computes the same set of complex events over streams. 
Then it is natural to ask whether this holds in the other direction, namely, if every MA or CEA can be translated into an equivalent formula with unary predicates.
If we restrict to core formulas, then the answer is no, mainly because MA and also CEA can take decisions based on tuples that are not part of the output match, while formulas in core formulas cannot.
As an example, consider again the CEA in Figure~\ref{fig:complement_CEA} that outputs all $H$-event where there exists no $T$-event afterwards. 
It is straightforward to prove that there is no unary core formula whose output is equivalent to the CEA defined above.

In order to capture the exact expressiveness of unary core formulas, we restrict CEA to a new semantics called the \emph{$*$-semantics}.
%The difference of the semantics is in the way the automaton runs.
Formally, let $\cA = (Q, \Delta, I, F)$ be a complex event automaton and $S=t_1,t_2,\ldots$ be a stream.
A $*$-run $\rho^*$ of $\cA$ over $S$ is a sequence of transitions:
$
\rho^*: (q_0,0) \ \trans{\alpha_1/L_1} \ (q_1,i_1) \  \trans{\alpha_2/L_2} \ \cdots \ \trans{\alpha_n/L_n} (q_n,i_n)
$
such that $q_0 \in I$, $0 < i_1 < \ldots < i_n$ and, for every $j \geq 1$, $(q_{j-1}, \alpha_j, L_j, q_j) \in \Delta$ with  $S[i_j] \models \alpha_j$ and $L_j \neq \emptyset$.
We say that $\rho^*$ is an accepting $*$-run if $q_n \in F$.
Furthermore, we denote by $C_\rho:\lset \rightharpoonup 2^\bbN$ the complex event induced by $\rho^*$ as $C_{\rho^*}(A) = \{i_j \mid A \in L_j\}$ and undefined if $A \notin L_i$ for every $i$.
The set of all matches of $\cA$ over $S$ under the $*$-semantics is defined as:
$
\ssem{\cA}(S) = \{C_{\rho^*} \mid \text{$\rho^*$ is an accepting $*$-run of $\cA$ over $S$}\}
$.
Notice that the automaton no longer has the ability to verify a condition on a tuple with an $\empty$-labeled position.
Indeed, one may eliminate the $\emptyset$-labeled transitions, i.e., consider $\Delta \subseteq Q \times \fset_u(\cR) \times (2^\lset- \{\emptyset\}) \times Q$.
For the sake of simplicity, we keep the syntax of CEA and just restrict its semantics instead of defining a new automata model.

%A basic property of this semantics is that for every MA $\cA$, there is another MA $\cA'$ such that $\sem{\cA}_*(S) = \sem{\cA'}(S)$ for every stream $S$.
%Basically, $\cA'$ is the result of adding the $\amark$ mark to every transition of $\cA$ and a loop with $\umark$ and $true$ condition for every state. Formally, if $\cA=(Q,\Delta,I,F)$ then $\cA'=(Q,\Delta',I,F)$ where $\Delta'=\{(p,(\alpha,\amark),q) \mid (p,\alpha,q)\in \Delta\} \cup \{(q,(true,\umark),q) \mid q\in Q \}$.

With the new semantics, we can effectively capture the expressiveness of unary core formulas as follows.
\begin{theorem} \label{theo:CEP_MA*}
	Unary core formulas are equally expressive as CEA under the $*$-semantics, namely, for every core formula $\varphi$ with unary predicates, there exists a CEA $\cA$ such that $\sem{\varphi}(S)=\ssem{\cA}(S)$ for every stream $S$, and conversely.
\end{theorem}
%The proof for the first part is similar to the one in section~\ref{section}. Basically, $\varphi$ is first translated into normal form and then the automaton $\cA$ is constructed recursively.
%The proof for the second part follows the same idea as the proof that FSA can be expressed as regular expressions.
%For the sake of saving space, the complete proof for Theorem~\ref{theo:CEP_MA*} has been moved to the appendix.

Theorem~\ref{theo:CEP_MA*} gives a useful result for understanding the expressiveness of unary core formulas.
Moreover, statements resulting from the study of CEA under $*$-semantics can be further applied to unary core formulas and conversely.
In this direction, an interesting property of the $*$-semantics is that, for every CEA $\cA$, stream $S$, and complex event $C \in \ssem{\cA}(S)$, we can arbitrarily modify, add or remove tuples in $S$ that are not \emph{marked} by~$C$, and the original tuples in $C$ would still make a match of~$\cA$ over the resulting stream.
To formalize this, we need some additional definitions.
A \emph{processing-function} $f$ is a function $f:\streams(\cR) \rightarrow 2^\cset$, where $\streams(\cR)$ is the set of all $\cR$-streams and $\cset$ is the set of all complex events (i.e. the set of all finite functions $C: \lset \rightharpoonup 2^\bbN$).
Although $f$ can be any function that returns set of complex events on input streams, we are interested in the processing-functions $f$ that can be described either by a core formula $\varphi$ (i.e. $f = \sem{\varphi}$) or by a CEA $\cA$ (i.e. $f = \sem{\cA}$).
Let $S_1$, $S_2$ be two streams and $C_1$, $C_2$ be two complex events.
We say that $S_1$ and $C_1$ are \emph{$*$-related} with $S_2$ and
$C_2$, written as $(S_1,C_1)=_*(S_2,C_2)$, if $S_1[C_1] = S_2[C_2]$
(recall that $S[C]$ is the subsequence of $S$ at the positions in
$C$).
\stijn{I don't think that the notation $S[C]$ has be introduced

  before. It suffices to define it here.}

Consider now any match-function $f$. We say that $f$ has the \emph{$*$-property} if, for every stream $S$ and any complex event $C \in f(S)$, it holds that $C' \in f(S')$ for every $S'$ and $C'$ such that $(S,C)=_*(S',C')$.
A way to understand the $*$-property is to see $S'$ as the result of fixing the tuples in $S$ that are part of $C$ (i.e. $S[C]$) and adding or removing tuples arbitrarily, and defining $C'$ to be the complex event that has the same original tuples of $C$. The following theorem states the relation that exists between the $*$-property and the $*$-semantics over CEA.

\begin{proposition} \label{prop:MA_MA*}
	If the processing-function defined by a CEA~$\cA$ has the $*$-property, then there exists a CEA $\cA'$ such that $\sem{\cA}(S) = \ssem{\cA'}(S)$ for every $S$.
\end{proposition}
By combining Theorem~\ref{theo:CEP_MA*} and Proposition~\ref{prop:MA_MA*} we get the following useful result that shows when a processing function can be defined by unary core formula.
\begin{corollary}\label{cor:CEPL*}
	Let $f$ be a processing function. Then $f$ can be defined by a complex event automaton and has the $*$-property if, and only if, there exists a unary core formula $\varphi$ such that $f = \sem{\varphi}$.
\end{corollary}

Many query languages for CEP have been proposed in the literature and most of them include the core  fragment presented in Section~\ref{sec:prelim}.
However, there are other useful operators that have been introduced in literature like $\scand$, $\scall$ and $\scunless$. These operators were also formally defined in~\cite{GRUpaper} and we give here its formal definition for the sake of completeness. Formally, given a complex event $C$, a stream $S$ and $i, j \in \bbN$:
\stijn{For the semantics of $\call$ below, $i$ and $j$ are supposed to
  be natural numbers, but are $\inf$ if $C_1$ or $C_2$ is the trivial match.}
\begin{itemize}
	\item $C \in \sem{\rho_1 \cand \rho_2}(S, i, j)$ iff $C \in \sem{\rho_1}(S,i,j) \cap \sem{\rho_2}(S,i,j)$.
	\item $C \in \sem{\rho_1 \call \rho_2}(S, i, j)$ iff there exist $i_1,i_2,j_1,j_2 \in \bbN$ and matches $C_1$, $C_2$ such that $M_k \in \sem{\rho_k}(S,i_k,j_k)$, $C = C_1 \cup C_2$, $i = \min\{i_1,i_2\}$ and $j = \max\{j_1,j_2\}$.
	\item $C \in \sem{\rho_1 \cunless \rho_2}(S, i, j)$ iff $C \in
          \sem{\rho_1}(S,i,j)$ and, for every complex event $C'$ and $i',j' \in \bbN$ such that $i \leq i' \leq j' \leq j$, it holds that $C' \notin \sem{\rho_2}(S,i',j')$.
\end{itemize}
Interestingly, the extended operators $\scand$ and $\scall$ were rather introduced in some papers since it seems that they are not strictly necessary in the core of CEPL. By using Corollary~\ref{cor:CEPL*}, we can easily understand this language decision, in the sense that $\scand$ and $\scall$ do not add expressive power to unary core-CEPL. Indeed, $\scand$ and $\scall$ can be defined by complex event automaton and both satisfy the $*$-property.

\begin{corollary} \label{cor:and_all}
	For every unary formula $\varphi$ of the form $\varphi_1~\OP~\varphi_2$, with $\OP \in \{\scand, \scall\}$ and $\varphi_i$ unary core formulas, there is a unary core formula $\varphi'$ such that $\sem{\varphi}(S) = \sem{\varphi'}(S)$ for every stream $S$.
\end{corollary}

Unfortunately, the $\scunless$-operator can be defined by CEA but one can easily show that there exist $\scunless$-formulas which do not satisfy the $*$-property. 
Consequently, by Corollary~\ref{cor:CEPL*} this formulas cannot be defined in unary core-CEPL.
This says that $\scunless$ adds expressibility to core formulas while remaining processable by the same computational model. Therefore, it makes sense to included in the design of a CEP query language.


% %%% Local Variables: 
% %%% mode: latex
% %%% TeX-master: "../main/main"
% %%% End: 


